Foundations for Unfairness in Anomaly Detection -- Case Studies in Facial Imaging Data

Deep anomaly detection (AD) is perhaps the most controversial of data analytic tasks as it identifies entities that are then specifically targeted for further investigation or exclusion. Also controversial is the application of AI to facial imaging data. This work explores the intersection of these two areas to understand two core questions: "Who" these algorithms are being unfair to and equally important "Why". Recent work has shown that deep AD can be unfair to different groups despite being unsupervised with a recent study showing that for portraits of people: men of color are far more likely to be chosen to be outliers. We study the two main categories of AD algorithms: autoencoder-based and single-class-based which effectively try to compress all the instances with those that can not be easily compressed being deemed to be outliers. We experimentally verify sources of unfairness such as the under-representation of a group (e.g. people of color are relatively rare), spurious group features (e.g. men are often photographed with hats), and group labeling noise (e.g. race is subjective). We conjecture that lack of compressibility is the main foundation and the others cause it but experimental results show otherwise and we present a natural hierarchy amongst them.

==> 03empirical.tex <==


\input{tables/summary_clustered}



Starting with the unbiased datasets containing an equal number of samples in each group and equal group base rates, we create different biased datasets by varying $\beta_s$, $\beta_u$, $\beta_v$ (or $\beta_m$), and $\beta_g$, depending on the type of bias being injected.
Note that we tune hyperparameters as described in \S\ref{ssec:methods} for each resulting dataset separately (see Apdx. \S\ref{asec:cluster_details} for details).


Table \ref{tab:summary} provides a qualitative summary of our findings across OD models and bias types \note{for datasets with clustered outliers. We discuss the detailed analysis as follows. (We provide a similar summary in Table \ref{tab:summary_scatter} for datasets with scattered outliers, along with detailed analysis of results in Apdx. \S\ref{asec:scatter_details} for brevity.)} 

\note{Overall, we see that the bias-injected group $b$ is impacted disproportionately  across models and bias types (with a few exceptions), although the severity varies.
Moreover, bias impacts not only fairness but also detection performance; in fact, there are cases when performance drops drastically despite little to no difference between groups.
}

\input{tables/summary_scattered}


\subsection{Group sample size bias}
\label{ssec:sizebias}


When samples from group $b$ are dropped at random, the inliers and outliers both sparsify relative to group $a$.
We find that {OD models react to density differences in the feature space  differently}. 
The stark contrast can be explained based on the modeling assumptions of these models, as they interact with density differences. 

As shown in Fig. \ref{fig:samplesize_lof_cluster}, LOF's flag rate for group $b$ drops, which in turn increases the FPR  while decreasing Precision for group $a$. In contrast, iForest behaves \textit{vice versa} as shown in Fig. \ref{fig:samplesize_if_cluster}.
LOF evaluates outlierness \textit{locally}, by comparing points to their neighbors. When group $b$ inliers sparsify, $b$-outliers ``hide'' better due to masking \cite{jiang2022d}. Isolation-based iForest, on the other hand, can more quickly isolate now-sparser points in group $b$, overly flagging them, hence maintaining high TRP, but larger FPR and lower Precision.
Note that iForest's brittleness is also evident from its overall performance falling more drastically with increasing bias.

DeepAE behaves similar to iForest (see Apdx. Fig. \ref{fig:samplesize_deepae_cluster}), although through a different mechanism. Since subsampling group $b$ renders them rare \textit{minority} samples, their impact on the total loss of the compression-based DeepAE diminishes. As a result, their poor reconstruction reflects as higher flag rate, larger FPR and lower Precision.  

%\note{remediation by SMOTE upsampling or counterfactual generation - }

%Disparity in sample sizes could be either due to imbalance in the underlying demographic distribution or it may be a result of data collection or sampling strategy.




\input{figures/samplesize_lof_cluster.tex}

\input{figures/samplesize_if_cluster.tex}



\subsection{Target under-representation bias}
\label{ssec:urep}

The algorithm outputs change considerably when exposed to the under-representation bias, where we only drop target (positive) samples from group $b$.
Note that removing outlier samples from $b$ renders group $a$'s observed base rate higher.

With a higher base rate, group $a$'s outliers are slightly masked, which reduces the TPR on $a$, while increasing TPR for $b$. FPR increases for both groups, proportionate to the overall increase, whereas Precision $b$ drops lower than that for $a$.
iForest is robust to masking as it can find cuts in the feature space that isolates the outlier clusters at once, and therefore, it retains high detection performance with little to no disparity between the groups. 
Similar to iForest, DeepAE also retains F1 performance above 0.9 across bias levels with no notable disparities between groups, mainly because dropping few outlier samples does not change the bulk of the data and the compression quality. 



\subsection{Feature measurement bias}
\label{ssec:meas}

Feature variance loosens the clusters and creates extreme-valued samples among both inliers and outliers in group $b$. As a result, LOF ranks group $a$ outliers strictly above those from group $b$ as they retain a starker contrast to their relative inliers. Beyond a certain noise level, LOF wrongly flags group $b$ inliers with lower TPR and Precision, while maintaining steady flag rate, TPR, FPR and Precision for $a$. 
iForest is more robust with only a slightly higher FPR and slightly lower TPR and Precision for group $b$, thus retaining high overall performance.   

DeepAE performance is affected considerably with TPR and Precision falling sharply, since half of the data is noisy and harder to compress, although the poor model fit impacts both groups similarly with no notable difference. We note this as a curious case where data bias significantly impacts model performance but not fairness.

\note{mean shift}


\subsection{Membership obfuscation bias}
\label{ssec:obf}

Different from earlier bias scenarios in which the data collector or their instrument may be inflicting the bias, here the individuals in the population themselves bias the data distribution. They do so by inducing mixed-up subpopulations, which resemble in some parts to group $b$ and in other parts to group $a$. As the obfuscation variables are randomized, this leads to \textit{multi-modality} within group $b$ with many small subpopulations.

LOF is extremely sensitive to this type of bias as it flags more and more of these small micro-clusters in group $b$ with increasing levels of bias; with reduced TPR for both groups, and high FPR and low Precision for group $b$. Its overall performance also drops considerably. 
iForest, on the other hand, is much more robust because it is \textit{subspace}-based; that is, it is able to isolate outliers as long as it makes axis-cuts on the culprit variables. Put differently, as long as it does not solely pick proxy variables, it does not wrongly flag group $b$ micro-clusters. The probability of such events is low, hence the slight unfairness against group $b$, with high overall performance retained. 
Similar to LOF's, DeepAE is sensitive to the presence of small micro-clusters as more variability in data patterns imply harder compression. Thus its overall performance drops, with higher flag rate, higher FPR and lower Precision for group $b$.


{\bf Remarks.~} Table \ref{tab:summary_scatter}

==> 04experiments.tex <==





%\subsection{Moving beyond ``Algorithmic bias is a data (bias) problem''}



When data from some protected groups is inflicted with data bias, it often leads to differences in the observed data distributions of the different groups.  
While this can be interpreted as a data bias problem, it is important to note that differences in data distributions between groups may as well be natural. %, organic data property. In other words, the differences or heterogeneities between groups introduced by various data biases may in fact be naturally exhibited by the original groups in the raw data in the first place.


In the following subsections, we aim to make connections between specific data properties that emerge as a result of bias and how such properties may also appear in the real world organically. 
These connections support the argument toward moving beyond the ``algorithmic bias is a data (bias) problem'' debate \cite{hooker2021moving}.
That is, algorithmic bias can arise solely from the interaction between  modeling assumptions and  certain properties the input data exhibits, without the data being necessarily inflicted with any bias. 


In a nutshell, group-wise differences in certain data properties (such as density, prevalence, multi-modality, etc.) -- either induced by data bias or  exhibited naturally -- could result in unfair outcomes. Whichever the source may be, it is useful to understand which OD algorithms are more prone to unfairness in the face of such group-wise differences, especially in scenarios where these differences can be quantified.



\subsection{Group Sample Size Bias mimics Density Heterogeneity among Groups}
\label{ssec:sizebias2}

In injecting group sample size bias,  
the act of downsampling data from one group creates a population that is sparsely sampled from the underlying manifold. 
This induces variable density in the feature space. We observed that this property makes isolation-based iForest brittle, as it  tends to more easily (yet mistakenly) isolate the samples in sparser regions. 

However, it may also be natural that different groups in fact exhibit different density distributions. This would be especially realistic for proxy variables. For example, it is easy imagine that hair length, which is a proxy for gender, would follow  distributions with varying density between groups. A similar argument can be made for income, which can be a proxy for race, with widely varying density distributions between groups.

%\note{introduce sparsity in $X_g$ only}

%\note{no sample size disparity, only density disparity in experiments -- loss-based detectors no longer prone to minority bias in the total loss (hence may behave differently: to be seen).}

\subsection{Target Under-Representation Bias mimics Base-Rate Heterogeneity among Groups}
\label{ssec:urep2}

$P(Y=1|G=a) \neq P(Y=1|G=b)$





\subsection{Feature Measurement Bias mimics  \\ Variance Heterogeneity among Groups}
\label{ssec:meas2}
Variance-shift reflecting measurement noise may change the propensity of extreme values as well as low-frequency observations.




\note{introduce variance difference in $X_g$ only; e.g. first name variability}



\subsection{Membership Obfuscation Bias mimics  Multi-modality within Groups}
\label{ssec:obf2}
not only distorts base-rates but also induces heterogeneous subpopulations









==> dfn.tex <==



\newsavebox\CBox
\def\textBF#1{\sbox\CBox{#1}\resizebox{\wd\CBox}{\ht\CBox}{\textbf{#1}}}


%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}
%\renewcommand{\algorithmiccomment}[1]{\hfill$\blacktriangleright$ #1}

\newcommand{\cdash}{\multicolumn{1}{c}{--} }


\newcommand{\super}{$^\blacktriangle$}
\newcommand{\sub}{$^\triangledown$}

\newcommand{\qap}{$\bm{q}_{\textbf{AP}}$}
\newcommand{\qroc}{$\bm{q}_{\textbf{ROC}}$}
\newcommand{\qprn}{$\bm{q}_{\textbf{Prec}}$}

%\newcommand{\methodtitle}{{\Large \sf FrAUDIT}\xspace}

%\newcommand{\methodtitle}{{\Large \sf SSTSAD}\xspace}

\newcommand{\method}{{\sf Bias Busted}\xspace}

%\DeclareMathAlphabet      {\mathbfit}{OML}{cmm}{b}{it}
\newcommand*{\bord}{\multicolumn{1}{c|}{}}

\newcommand{\cbit}{\begin{compactitem}}
	\newcommand{\ceit}{\end{compactitem}}
\newcommand{\cben}{\begin{compactenum}}
	\newcommand{\ceen}{\end{compactenum}}

\definecolor{OliveGreen}{rgb}{0,0.6,0}
\newcommand{\tick}{\textcolor{OliveGreen}{\ding{52}}}

\newcommand{\bit}{\begin{itemize}}
	\newcommand{\eit}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
	\newcommand{\een}{\end{enumerate}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}


\newcommand{\ap}{AP\xspace}
\newcommand{\roc}{ROC\xspace}
\newcommand{\pre}{Prec@$k$\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%10 measures
\newcommand{\std}{{\sc std}\xspace}
%\newcommand{\rs}{{\sc rs}\xspace}
\newcommand{\h}{{\sc h}\xspace}
\newcommand{\ch}{{\sc ch}\xspace}
\newcommand{\iind}{{\sc i}\xspace}
\newcommand{\dunn}{{\sc d}\xspace}
\newcommand{\s}{{\sc s}\xspace}
\newcommand{\db}{{\sc db}\xspace}
\newcommand{\xb}{{\sc xb}\xspace}
\newcommand{\sd}{{\sc sd}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Goix - EM / MV
\newcommand{\emmes}{{\sc EM}\xspace}
\newcommand{\mv}{{\sc MV}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%ireos
\newcommand{\ireos}{{\sc IREOS}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Consensus
\newcommand{\udr}{{\sc UDR}\xspace}
\newcommand{\mc}{{\sc MC}\xspace}
\newcommand{\mcs}{{\sc MC$_S$}\xspace}

\newcommand{\hits}{{\sc HITS}\xspace}
\newcommand{\ens}{{\sc Ens}\xspace}

\newcommand{\hitsc}{{\sc HITS-auth}\xspace}
\newcommand{\ensc}{{\sc Ens-pseudo}\xspace}
\newcommand{\hitscs}{{\sc HITS-au}\xspace}
\newcommand{\enscs}{{\sc Ens-pse}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\rand}{{\sc Random}\xspace}
\newcommand{\ifor}{{\sc iForest-r}\xspace}

\newcommand{\rnd}{{\sc Rnd}\xspace}
\newcommand{\ifr}{{\sc iF}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\best}{{\sc Best}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%



\newcommand{\Xg}{\mathcal{X}_g}
\newcommand{\Xc}{\mathcal{X}_c}
\newcommand{\Xo}{\mathcal{X}_o}

\newcommand{\bX}{\bold{X}}
\newcommand{\bx}{\bold{x}}
\newcommand{\bs}{\bold{s}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bchi}{\boldsymbol{\chi}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}

\newcommand{\todo}[1]{{\textsf{\textcolor{red}{[TODO: #1]}}}}
\newcommand{\note}[1]{{\textsf{\textcolor{blue}{[#1]}}}}
\newcommand{\summary}[1]{{\textsf{\textcolor{red}{#1}}}}

\newcommand{\hide}[1]{}

\newtheorem{problem}{Problem}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/summary_clustered.tex <==

\definecolor{armygreen}{rgb}{0.0, 0.5, 0.0}

\begin{table}[!t]
%	\setlength{\tabcolsep}{3pt}
	\caption{
 Qualitative summary of results for fairness stress-testing  of various OD algorithms (columns) when different type data bias (rows) is applied on group $b$ with \underline{clustered} outliers. 
 \underline{Shades of colors} \textcolor{red}{red} and \textcolor{blue}{blue} depict the degree of \underline{\textit{unfairness}}, when disproportionately  inflicted on group \textcolor{red}{$a$} or group \textcolor{blue}{$b$}, respectively; blank implying no notable difference. % is in {\textcolor{armygreen!80}{green}}.
 \underline{Arrow counts} reflect relative change in overall detection \underline{\textit{performance}}; no arrows implying no notable change.} 	
			\vspace{-0.1in}
			\begin{tabular}{l|p{1.05cm}|p{1.05cm}|p{1.05cm}|l} 
				\toprule
    Bias type / OD model   &
    	{LOF} & 
     {iForest} & 
     {DeepAE} & 
     FairOD  \\
       \midrule

       Sample size (\S\ref{ssec:sizebias})  
       & \cellcolor{red!30}   \centering $\downarrow$
       & \cellcolor{blue!70} \centering $\downarrow\downarrow$
       &  \cellcolor{blue!30} \centering $\downarrow$
       &   \\ \hline
       Under-rep. (\S\ref{ssec:urep})   
       &  \cellcolor{blue!20} \centering $\downarrow$
       &  %\cellcolor{armygreen!50}
       &   \cellcolor{blue!10}
       %\centering 
       &    \\ 
       \hline
       Measurement (\S\ref{ssec:meas})  
       &  \cellcolor{blue!40} \centering $\downarrow$
       &  \cellcolor{blue!20}
       &  %\cellcolor{armygreen!50} 
       &  \\ 
       \hline
       Obfuscation (\S\ref{ssec:obf})  
       & \cellcolor{blue!70} \centering $\downarrow\downarrow\downarrow$    
       & \cellcolor{blue!40} \centering $\downarrow$
       & \cellcolor{blue!70} \centering 
 $\downarrow\downarrow$  
        &  \\ 
         \bottomrule
       \end{tabular}

       \label{tab:summary}
	\vspace{-0.15in}
\end{table}

==> tables/summary_scattered.tex <==

\definecolor{armygreen}{rgb}{0.0, 0.5, 0.0}

% \cellcolor{red!30}   \centering $\downarrow$
% \cellcolor{blue!70} 
% \cellcolor{armygreen!50}

\begin{table}[!th]
%	\setlength{\tabcolsep}{3pt}
	\caption{
Qualitative summary of results for fairness stress-testing  of various OD algorithms (columns) when different type data bias (rows) is applied on group $b$ with \underline{scattered} outliers. 
 Shades of \textcolor{red}{red} and \textcolor{blue}{blue} depict the degree of \textit{unfairness}, if disproportionately  inflicted on group \textcolor{red}{$a$} or group \textcolor{blue}{$b$}, respectively; blank implying no notable difference. 
 Arrows reflect the relative change in detection \textit{performance}; no arrows implying no notable change.} 	
			\vspace{-0.1in}
			\begin{tabular}{l|p{1.05cm}|p{1.05cm}|p{1.05cm}|l} 
				\toprule
    Bias type / OD model   &
    	{LOF} & 
     {iForest} & 
     {DeepAE} & 
     FairOD  \\
       \midrule

       Sample size (\S\ref{assec:sizebias_scatter})  
       & \cellcolor{red!30} 
       & \cellcolor{blue!70} \centering $\downarrow\downarrow$
       &  %\cellcolor{armygreen!50}
       &   \\ \hline
       Under-rep. (\S\ref{assec:urep_scatter})   
       &  \cellcolor{blue!10}
       &  \cellcolor{blue!20}
       &  \cellcolor{blue!10}
       &  \\ 
       \hline
       Measurement (\S\ref{assec:meas_scatter})  
       &  \cellcolor{blue!70} \centering $\downarrow\downarrow$
       &  \cellcolor{blue!50} \centering $\downarrow$
       &  \cellcolor{blue!60} \centering $\downarrow\downarrow$
       &  \\ 
       \hline
       Obfuscation (\S\ref{assec:obf_scatter})  
       & \cellcolor{blue!30} \centering $\downarrow$  
       & \cellcolor{blue!40} \centering $\downarrow$
       & \cellcolor{blue!70} 
       \centering $\downarrow\downarrow$ 
       &  \\ 
         \bottomrule
       \end{tabular}

       \label{tab:summary_scatter}
	\vspace{-0.15in}
\end{table}
